Effective interface conditions for the forced infiltration of a viscous fluid into a porous medium using homogenization

It is generally accepted that the effective velocity of a viscous flow over a porous bed satisfies the Beavers-Joseph slip law. To the contrary, in the case of a forced infiltration of a viscous fluid into a porous medium the interface law has been a subject of controversy. In this paper, we prove rigorously that the effective interface conditions are: (i) the continuity of the normal effective velocities; (ii) zero Darcy's pressure and (iii) a given slip velocity. The effective tangential slip velocity is calculated from the boundary layer and depends only on the pore geometry. In the next order of approximation, we derive a pressure slip law. An independent confirmation of the analytical results using direct numerical simulation of the flow at the microscopic level is given, as well.

==> preamble.tex <==
    \usepackage{graphicx}
    \usepackage[autolanguage]{numprint}
\usepackage{hyperref}
\usepackage{booktabs} % for much better looking tables
\usepackage{fixmath,amsmath,amssymb,amsfonts}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\usepackage{natbib}
\usepackage{subfig}
\usepackage{float}
\newcommand{\e}{{{\epsilon}}}
\newcommand{\eff}{{{\text{eff}}}}

\newcommand {\ueff}{\ensuremath{\mathbf{u}^\eff}}
\newcommand {\peff}{\ensuremath{{p}^\eff}}
\newcommand {\pnull}{\ensuremath{{P}^D}}

\newcommand{\ve}{\ensuremath{{\v}^\epsilon}}
\newcommand{\vecomp}[1]{\ensuremath{{v}_{#1}^\epsilon}}
\newcommand{\pe}{\ensuremath{p^\epsilon}}

\newcommand{\betabl}[1][2]{\ensuremath{\boldsymbol \beta^{bl,#1}}}
\newcommand{\omegabl}[1][2]{\ensuremath{\omega^{bl,#1}}}

\newcommand{\cbl}{\ensuremath{C^{2,bl}_1}}
\newcommand{\cblpi}{\ensuremath{C^{2}_\pi}}

